Boosting Vision-Language Models for Histopathology Classification: Predict all at once

The development of vision-language models (VLMs) for histo-pathology has shown promising new usages and zero-shot performances. However, current approaches, which decompose large slides into smaller patches, focus solely on inductive classification, i.e., prediction for each patch is made independently of the other patches in the target test data. We extend the capability of these large models by introducing a transductive approach. By using text-based predictions and affinity relationships among patches, our approach leverages the strong zero-shot capabilities of these new VLMs without any additional labels. Our experiments cover four histopathology datasets and five different VLMs. Operating solely in the embedding space (i.e., in a black-box setting), our approach is highly efficient, processing $10^5$ patches in just a few seconds, and shows significant accuracy improvements over inductive zero-shot classification. Code available at https://github.com/FereshteShakeri/Histo-TransCLIP.

==> tables/results.tex <==
\begin{table*}[ht] 
\footnotesize
\centering
\renewcommand{\arraystretch}{1.05}
    \caption{Zero-shot and Histo-TransCLIP performance on top of various VLMs. Best values are highlighted in \textbf{bold}. \textcolor{DarkGreen}{\textbf{$\Delta_{\text{transductive}}$}} is the average accuracy gain brought by our transductive approach.}
    \label{table:mainresult}
    \vspace{0.1cm}
\begin{tabular}{llccccc}
\toprule
 Dataset & Method & \multicolumn{5}{c}{Model}\\
\midrule
\midrule
&  & CLIP& Quilt-B16 & Quilt-B32 & PLIP & CONCH \\
\midrule
\multirow{2}{*}{\textit{SICAP-MIL}} & Zero-shot & \textbf{29.85} & 40.44 & \textbf{35.04} & 46.84 & 27.71  \\
 & \cellcolor{LightBlue} Histo-TransCLIP & \cellcolor{LightBlue} 24.72 & \cellcolor{LightBlue} \textbf{58.49} & \cellcolor{LightBlue} 28.18 & \cellcolor{LightBlue} \textbf{53.23} & \cellcolor{LightBlue} \textbf{32.58}  \\
\midrule
\multirow{2}{*}{\textit{LC(Lung)}} & Zero-shot & \textbf{31.46} & 43.00 & 76.24 &  84.96 & 84.81  \\
 & \cellcolor{LightBlue} Histo-TransCLIP & \cellcolor{LightBlue} 25.62 & \cellcolor{LightBlue} \textbf{50.53} & \cellcolor{LightBlue} \textbf{93.93} & \cellcolor{LightBlue} \textbf{93.80} & \cellcolor{LightBlue} \textbf{96.29} \\
\midrule
\multirow{2}{*}{\textit{SKINCANCER}} & Zero-shot & 4.20 & 15.38 & 39.71 & 22.90 & 58.53  \\
& \cellcolor{LightBlue} Histo-TransCLIP & \cellcolor{LightBlue} \textbf{11.46} & \cellcolor{LightBlue} \textbf{33.33} & \cellcolor{LightBlue} \textbf{48.80} & \cellcolor{LightBlue} \textbf{36.72} & \cellcolor{LightBlue} \textbf{66.22}  \\
\midrule
\multirow{2}{*}{\textit{NCT-CRC}} & Zero-shot & 25.39 & 29.61 &  53.73 & 63.17 & 66.27  \\
& \cellcolor{LightBlue} Histo-TransCLIP & \cellcolor{LightBlue} \textbf{39.61} & \cellcolor{LightBlue} \textbf{48.40} & \cellcolor{LightBlue} \textbf{58.13} &  \cellcolor{LightBlue} \textbf{77.53} & \cellcolor{LightBlue} \textbf{70.36}  \\
\midrule
\multirow{3}{*}{\textit{Average}} & Zero-shot &  22.73 & 32.1 &  51.18 & 54.47 & 59.33 \\
& \cellcolor{LightBlue} Histo-TransCLIP &  \cellcolor{LightBlue} \textbf{25.35} & \cellcolor{LightBlue} \textbf{47.69} & \cellcolor{LightBlue} \textbf{57.26} & \cellcolor{LightBlue} \textbf{65.32} & \cellcolor{LightBlue} \textbf{66.36} \\
&  \textcolor{DarkGreen}{\textbf{$\Delta_{\text{transductive}}$}} & \textcolor{DarkGreen}{\textbf{+2.62}} & \textcolor{DarkGreen}{\textbf{+15.59}} & \textcolor{DarkGreen}{\textbf{+6.08}} & \textcolor{DarkGreen}{\textbf{+10.85}} & \textcolor{DarkGreen}{\textbf{+7.03}}\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/runtime.tex <==
\begin{table}[t]
    \centering
        \caption{Features denotes the runtime to pre-compute the image and text embeddings, Histo-TransCLIP denotes the runtime of our transductive procedure once embeddings are provided. Experiments were conducted on a single NVIDIA GeForce RTX 3090 (24Gb) GPU.}
    \label{tab:runtime}
    \vspace{0.1cm}
    \begin{tabular}{ccc}
        \toprule
         \#Patches & Features & Histo-TransCLIP \\
        \midrule
          $10^2$ & $\sim$ 1 sec. & $\sim$ 0.1 sec.\\
          $10^3$ & $\sim$ 4 sec. & $\sim$ 0.2 sec.\\
          $10^4$ & $\sim$ 28 sec. & $\sim$ 0.4 sec.\\
          $10^5$ & $\sim$ 5 min. & $\sim$ 6 sec.\\
         \bottomrule
       
    \end{tabular}
\end{table}
